Will solid-state drives accelerate your bioinformatics? In-depth profiling, performance analysis, and beyond

A wide variety of large-scale data has been produced in bioinformatics. In response, the need for efficient handling of biomedical big data has been partly met by parallel computing. However, the time demand of many bioinformatics programs still remains high for large-scale practical uses due to factors that hinder acceleration by parallelization. Recently, new generations of storage devices have emerged, such as NAND flash-based solid-state drives (SSDs), and with the renewed interest in near-data processing, they are increasingly becoming acceleration methods that can accompany parallel processing. In certain cases, a simple drop-in replacement of hard disk drives (HDDs) by SSDs results in dramatic speedup. Despite the various advantages and continuous cost reduction of SSDs, there has been little review of SSD-based profiling and performance exploration of important but time-consuming bioinformatics programs. For an informative review, we perform in-depth profiling and analysis of 23 key bioinformatics programs using multiple types of devices. Based on the insight we obtain from this research, we further discuss issues related to design and optimize bioinformatics algorithms and pipelines to fully exploit SSDs. The programs we profile cover traditional and emerging areas of importance, such as alignment, assembly, mapping, expression analysis, variant calling, and metagenomics. We explain how acceleration by parallelization can be combined with SSDs for improved performance and also how using SSDs can expedite important bioinformatics pipelines, such as variant calling by the Genome Analysis Toolkit (GATK) and transcriptome analysis using RNA sequencing (RNA-seq). We hope that this review can provide useful directions and tips to accompany future bioinformatics algorithm design procedures that properly consider new generations of powerful storage devices.

==> table_tools.tex <==
%---------------------------------------------------------------------
\begin{table*}[!t]
\processtable{List of the twenty three bioinformatics programs profiled and analyzed in this work\label{t:tool_list}}
{\scriptsize
\begin{tabular}{llllll}
\toprule %inserts double horizontal lines
& Name  &Task &Main algorithm& Source & Speedup$^\dagger$\\ % inserts table
%heading
\midrule % inserts single horizontal line
\gyes & GATK BaseRecal & Base quality recalibration& generates recalibration table based on covariates & \citealp{mckenna2010genome} & 78.4 \\
 & Samtools  &Utility tool& sorting, merging, indexing large sequence alignment& \citealp{li2009sequence} & 77.2 \\
 & ABySS  & NGS assembler& distributed de Bruijn graph, hash table searching &\citealp{simpson2009abyss} & 51.7\\
 & Cluster3 &  Microarray analsysis& calculating pairwise sequence distance, clustering& \citealp{de2004open} & 50.0\\
 & Blat  &  Sequence alignment & index searching on non-overlapping k-mers& \citealp{kent2002blat}& 23.6 \\
 & Reptile & NGS denoising& MSA with Hamming distance, k-spectrum extraction& \citealp{yang2010reptile}  & 13.7\\
 & GATK Aligner & Sequence realignment&Smith-Waterman local realignment&\citealp{mckenna2010genome} & 12.6\\
 & Maq & NGS assembler& ungapped sequence alignment, maximizing posterior probability& \citealp{li2008mapping} & 10.1\\
 & Tophat & RNA-seq analysis&segmented sequence alignment using Bowtie& \citealp{trapnell2009tophat} & 3.2\\
 & MC-UPGMA& Microarray analsysis& memory-constrained multi-round hierarchical clustering& \citealp{loewenstein2008efficient}  &2.7\\
\midrule %inserts single line
\gno & BWA &  Sequence alignment&Burrows-Wheeler transform, trie traversal& \citealp{li2009fast} &1.09\\
 & Blast & Sequence alignment&seed-based local sequence alignment& \citealp{altschul1990basic} & 1.08\\
 & ClustalW & Sequence alignment&multiple sequence alignment using NJ guide tree& \citealp{thompson1994clustal}& 1.06\\
 & GATK Unified &Genome variant calling& Bayesian likelihood modeling& \citealp{mckenna2010genome} & 1.05\\
 & GATK PrintReads &Utility tool&sorting, and merging sequence alignments& \citealp{mckenna2010genome} & 1.03\\
 & Scripture &RNA-seq analysis&sequence alignment using TopHat, graph traversal& \citealp{guttman2010ab} & 1.02\\
 & IGVtools &Utility tool&sequence alignment indexing, sorting& \citealp{robinson2011integrative} & 1.02\\
 & Meme &Motif finding&expectation-maximization, greedy search& \citealp{bailey2006meme} & 1.00\\
 & Bowtie 2 &Sequence alignment&Burrows-Wheeler-based sequence alignment& \citealp{langmead2012fast} & 1.00\\ % inserting body of the table
 & Mosdi &Motif finding&HMM-based statistical modeling, suffix tree traversal& \citealp{marschall2009efficient} & 1.00\\
 & AmpliconNoise &NGS denoising&Needleman-Wunsch, hierarchical clustering, EM& \citealp{quince2011removing} &1.00\\
 & Weeder &Motif finding&suffix tree-based exhaustive searching& \citealp{pavesi2007weederh} & 1.00\\
 & ErmineJ &Microarray analsysis&permutation, rank-based statistics analysis& \citealp{gillis2010gene} &0.97\\
\botrule
\end{tabular}
}{\gyes, programs with 2x or more speedup; \gno, programs with negligible improvements; MSA, multiple sequence alignment; NJ, neighbor joining; HMM, hidden Markov model; EM, expectation maximization; $\dagger$ speedup by Intel 520 SSD over Seagate Barracuda HDD [see Tables~\ref{t:ssd_spec} and \ref{t:hdd_spec} for specifications and Table~\ref{t:data_list} for input data].}


\end{table*}
%---------------------------------------------------------------------

